Toward CUPID-1T

Current experiments to search for broken lepton-number symmetry through the observation of neutrinoless double-beta decay ($0\mathrm{\nu\beta\beta}$) provide the most stringent limits on the Majorana nature of neutrinos and the effective Majorana neutrino mass ($m_{\beta\beta}$). The next-generation experiments will focus on the sensitivity to the $0\mathrm{\nu\beta\beta}$ half-life of $\mathcal{O}(10^{27}$--$10^{28}$~years$)$ and $m_{\beta\beta}\lesssim15$~meV, which would provide complete coverage of the so-called Inverted Ordering region of the neutrino mass parameter space. By taking advantage of recent technological breakthroughs, new, future calorimetric experiments at the 1-ton scale can increase the sensitivity by at least another order of magnitude, exploring the large fraction of the parameter space that corresponds to the Normal neutrino mass ordering. In case of a discovery, such experiments could provide important insights toward a new understanding of the mechanism of $0\mathrm{\nu\beta\beta}$. We present here a series of projects underway that will provide advancements in background reduction, cryogenic readout, and physics searches beyond $0\mathrm{\nu\beta\beta}$, all moving toward the next-to-next generation CUPID-1T detector.

==> BeyondNDBD_ExoticNeutrinoStudies/BeyondNDBD_ExoticNeutrinoStudies.tex <==
% Topics: Neutrino magnetic moment, Sterile neutrinos

\subsubsection{Neutrino Magnetic Moment} \label{sec:NuMagneticMoment}
Lithium / neutrino source
\subsubsection{Sterile Neutrino Searches} \label{sec:SterileNuSearches}
\subsubsection{CEvNS} \label{sec:CEvNS}
\pingem{Benjamin Schmidt \ric}


==> BroaderImpacts/BI_NuclearPhysics.tex <==
This is the classification for \ndbd{}; we start with this.  We gain new information on nuclear decays, and by measuring the two neutrino spectrum (as described above), we could potentially gain information on the nuclear matrix elements. 


\begin{figure}
    \centering
    \includegraphics[width=.6\textwidth]{BroaderImpacts/CUPID-dim7dim9.pdf}
    \caption{\textcolor{blue}{(FROM DOE PROPOSAL) Discovery sensitivity for a selected set of next-generation ton-scale experiments to dim-7 and dim-9 operators. Note that in this model, increasing sensitivity moves up towards larger $\Lambda$. The NMEs are taken from [44, 58], and correspond to the different colors. Only one point is drawn for the various CUPID scenarios because no NME computed with the Nuclear Shell Model is available for 100Mo. The input parameters for all experiments are the same as used for Fig. \ref{fig:2019sensandparam}}}
    \label{fig:NuclearPhysics_Dim7Dim9}
\end{figure}

==> CupidGroupOfInterestAuthors.tex <==
\noindent
K.~Alfonso\textsuperscript{1}, T.~Andrii\textsuperscript{2}, A.~Armatol\textsuperscript{3}, E.~Armengaud\textsuperscript{3}, W.~Armstrong\textsuperscript{4}, C.~Augier\textsuperscript{5}, F.~T.~Avignone~III\textsuperscript{6}, O.~Azzolini\textsuperscript{2}, A.~Barabash\textsuperscript{7}, A.~Barresi\textsuperscript{8}, D.~Baudin\textsuperscript{3}, F.~Bellini\textsuperscript{9,10}, G.~Benato\textsuperscript{11}, M.~Beretta\textsuperscript{12}, L.~Berg\'e\textsuperscript{14}, M.~Biassoni\textsuperscript{8}, J.~Billard\textsuperscript{5}, V.~Boldrini\textsuperscript{15,16}, C.~Bourgeois\textsuperscript{14}, A.~Branca\textsuperscript{8}, C.~Brofferio\textsuperscript{8}, C.~Bucci\textsuperscript{11}, A.~Caminata\textsuperscript{17,18}, L.~Canonica\textsuperscript{11}, S.~Capelli\textsuperscript{8}, L.~Cappelli\textsuperscript{11}, V.~Caracciolo\textsuperscript{11}, L.~Cardani\textsuperscript{9}, P.~Carniti\textsuperscript{8}, N.~Casali\textsuperscript{9}, A.~Cazes\textsuperscript{5}, C.~Chang\textsuperscript{4}, M.~Chapellier\textsuperscript{14}, A.~Charrier\textsuperscript{3}, D.~Chiesa\textsuperscript{8}, M.~Clemenza\textsuperscript{8}, I.~Colantoni\textsuperscript{9,19}, F.~Collamati\textsuperscript{20}, S.~Copello\textsuperscript{11}, F.~Cova\textsuperscript{8}, O.~Cremonesi\textsuperscript{8}, R.~J.~Creswick\textsuperscript{6}, A.~Cruciani\textsuperscript{9}, A.~D'Addabbo\textsuperscript{11}, G.~D'Imperio\textsuperscript{9,10}, I.~Dafinei\textsuperscript{9,10}, F.~Danevich\textsuperscript{21}, M.~de~Combarieu\textsuperscript{3}, M.~De~Jesus\textsuperscript{5}, P.~de~Marcillac\textsuperscript{14}, S.~Dell'Oro\textsuperscript{22}, S.~Di~Domizio\textsuperscript{17,18}, T.~Dixon\textsuperscript{12}, V.~Dompe\textsuperscript{11,23}, A.~Drobizhev\textsuperscript{13}, L.~Dumoulin\textsuperscript{14}, G.~Fantini\textsuperscript{11}, M.~Fasoli\textsuperscript{8}, M.~Faverzani\textsuperscript{8}, E.~Ferri\textsuperscript{8}, F.~Ferri\textsuperscript{3}, F.~Ferroni\textsuperscript{11,23}, E.~Figueroa-Feliciano\textsuperscript{24}, J.~Formaggio\textsuperscript{25}, A.~Franceschi\textsuperscript{26}, S.~Fu\textsuperscript{27}, B.~K.~Fujikawa\textsuperscript{13}, J.~Gascon\textsuperscript{5}, A.~Giachero\textsuperscript{8}, L.~Gironi\textsuperscript{8}, A.~Giuliani\textsuperscript{14}, P.~Gorla\textsuperscript{11}, C.~Gotti\textsuperscript{8}, P.~Gras\textsuperscript{3}, M.~Gros\textsuperscript{3}, E.~Guerard\textsuperscript{14}, T.~D.~Gutierrez\textsuperscript{28}, K.~Han\textsuperscript{29}, E.~Hansen\textsuperscript{12}, W.~He\textsuperscript{27}, K.~M.~Heeger\textsuperscript{30}, D.~Helis\textsuperscript{3}, H.~Z.~Huang\textsuperscript{31,1}, R.~G.~Huang\textsuperscript{12,13}, J.~Johnston\textsuperscript{25}, A.~Juillard\textsuperscript{5}, G.~Karapetrov\textsuperscript{32}, G.~Keppel\textsuperscript{2}, H.~Khalife\textsuperscript{14}, V.~Kobychev\textsuperscript{21}, Yu.~G.~Kolomensky\textsuperscript{12,13}, S.~Konovalov\textsuperscript{7}, C.~Li\textsuperscript{12}, P.~Loaiza\textsuperscript{14}, L.~Ma\textsuperscript{27}, M.~Madhukuttan\textsuperscript{14}, F.~Mancarella\textsuperscript{15,16}, R.~Mariam\textsuperscript{14}, L.~Marini\textsuperscript{12}, S.~Marnieros\textsuperscript{14}, M.~Martinez\textsuperscript{33}, R.~H.~Maruyama\textsuperscript{30}, B.~Mauri\textsuperscript{3}, D.~Mayer\textsuperscript{25}, Y.~Mei\textsuperscript{13}, S.~Milana\textsuperscript{20}, D.~Misiak\textsuperscript{5}, N.~Moggi\textsuperscript{15,34}, S.~Morganti\textsuperscript{9}, T.~Napolitano\textsuperscript{26}, M.~Nastasi\textsuperscript{8}, X.~F.~Navick\textsuperscript{3}, J.~Nikkel\textsuperscript{30}, S.~Nisi\textsuperscript{11}, C.~Nones\textsuperscript{3}, E.~B.~Norman\textsuperscript{12,13}, V.~Novosad\textsuperscript{4}, I.~Nutini\textsuperscript{8}, T.~O'Donnell\textsuperscript{22}, G.~Olivier\textsuperscript{14}, E.~Olivieri\textsuperscript{14}, C.~Oriol\textsuperscript{14}, J.~L.~Ouellet\textsuperscript{25}, S.~Pagan\textsuperscript{30}, C.~Pagliarone\textsuperscript{11}, L.~Pagnanini\textsuperscript{11}, M.~Pallavicni\textsuperscript{17,18}, P.~Pari\textsuperscript{3}, L.~Pattavina\textsuperscript{11}, B.~Paul\textsuperscript{3}, M.~Pavan\textsuperscript{8}, J.~Pearson\textsuperscript{4}, H.~Peng\textsuperscript{31}, G.~Pessina\textsuperscript{8}, V.~Pettinacci\textsuperscript{9,10}, C.~Pira\textsuperscript{2}, S.~Pirro\textsuperscript{11}, D.~Poda\textsuperscript{14}, T.~Polakovic\textsuperscript{4}, O.~Polischuk\textsuperscript{21}, S.~Pozzi\textsuperscript{8}, E.~Previtali\textsuperscript{8}, A.~Puiu\textsuperscript{11}, T.~Redon\textsuperscript{14}, D.~Reynet\textsuperscript{14}, R.~Rizzoli\textsuperscript{15,16}, C.~Rosenfeld\textsuperscript{6}, C.~Rusconi\textsuperscript{6},  V.~Sanglard\textsuperscript{5}, J.~Scarpaci\textsuperscript{14}, K.~Schaffner\textsuperscript{11}, B.~Schmidt\textsuperscript{24,13}, Y.~Shen\textsuperscript{27}, V.~Shlegel\textsuperscript{35}, V.~Singh\textsuperscript{12}, M.~Sisti\textsuperscript{8}, D.~H.~Speller\textsuperscript{36,30}, P.~T.~Surukuchi\textsuperscript{30}, L.~Taffarello\textsuperscript{37}, O.~Tellier\textsuperscript{3}, C.~Tomei\textsuperscript{9,10},
J.~Torres\textsuperscript{30},
V.~Tretyak\textsuperscript{21}, A.~Vedda\textsuperscript{8}, M.~Velazquez\textsuperscript{38}, K.~Vetter\textsuperscript{12}, S.~L.~Wagaarachchi\textsuperscript{12}, G.~Wang\textsuperscript{4}, B.~Welliver\textsuperscript{13}, J.~Wilson\textsuperscript{6}, K.~Wilson\textsuperscript{6}, L.~A.~Winslow\textsuperscript{25}, M.~Xue\textsuperscript{31}, V.~Yefremenko\textsuperscript{4}, V.~Yumatov\textsuperscript{7}, M.~Zarytskyy\textsuperscript{21}, J.~Zhang\textsuperscript{4}, A.~Zolotarova\textsuperscript{14}, S.~Zucchelli\textsuperscript{15,34}

\vspace{4mm}

\noindent
$^{1}$ University of California, Los Angeles, Los Angeles, CA, USA\\
$^{2}$ INFN Laboratori Nazionali di Legnaro, Legnaro, Italy\\
$^{3}$ French Alternative Energies and Atomic Energy Commission Fundamental Research Division, Saclay, France\\
$^{4}$ Argonne National Laboratory, Argonne, IL, USA\\
$^{5}$ Institut de Physique Nucl\'eaire de Lyon, Lyon, France\\
$^{6}$ University of South Carolina, Columbia, SC, USA\\
$^{7}$ Institute for Theoretical and Experimental Physics, Moscow, Russia\\
$^{8}$ INFN Sezione di Milano Bicocca and University of Milano Bicocca, Milano, Italy\\
$^{9}$ INFN Sezione di Roma, L'Aquila, Italy\\
$^{10}$ Sapienza University of Rome, Rome, Italy\\
$^{11}$ INFN Laboratori Nazionali del Gran Sasso, Assergi (AQ), Italy\\
$^{12}$ University of California, Berkeley, Berkeley, CA, USA\\
$^{13}$ Lawrence Berkeley National Laboratory, Berkeley, CA, USA\\
$^{14}$ Centre de Sciences Nucl\'eaires et de Sciences de la Mat\`ere, Orsay, France\\
$^{15}$ INFN Sezione di Bologna, Bologna, Italy\\
$^{16}$ CNR-Institute for Microelectronics and Microsystems, Bologna, Italy\\
$^{17}$ INFN Sezione di Genova, Genova, Italy\\
$^{18}$ University of Genova, Genova, Italy\\
$^{19}$ CNR-Institute of Nanotechnology, Rome, Italy\\
$^{20}$ INFN Sezione di Roma and Sapienza University of Rome, Rome, Italy\\
$^{21}$ Kiev Institute for Nuclear Resarch, Kiev, Ukraine\\
$^{22}$ Virginia Polytechnic Institute and State University, Blacksburg, VA, USA\\
$^{23}$ xo Science Institute, L'Aquila, Italy\\
$^{24}$ Northwestern University, Evanston, IL, USA\\
$^{25}$ Massachusetts Institute of Technology, Cambrige, MA, USA\\
$^{26}$ INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{27}$ Fudan University, Shanghai, China\\
$^{28}$ California Polytechnic State University, San Luis Obispo, CA, USA\\
$^{29}$ Shanghai Jiao Tong University, Shanghai, China\\
$^{30}$ Yale University, New Haven, CT, USA\\
$^{31}$ University of Science and Technology of China, Hefei, China\\
$^{32}$ Drexel University, Philadelphia, PA, USA\\
$^{33}$ University of Zaragoza, Zaragoza, Spain\\
$^{34}$ University of Bologna, Bologna, Italy\\
$^{35}$ Nikolaev Institute of Inorganic Chemistry, Novosibirk, Russia\\
$^{36}$ Johns Hopkins University, Baltimore, MD, USA\\
$^{37}$ INFN Sezione di Padova, Padova, Italy\\
$^{38}$ Laboratoire de Science et Ing\'enierie des Mat\'eriaux et Proc\'ed\'es, Grenoble, France\\

==> RD_MUX_DEMETER/DEMETER_quantum.tex <==
The next generation of quantum computers and superconducting qubit instruments must be operated in cryogenic infrastructure \cite{the_national_academies_of_sciences_engineering_and_medicine_quantum_2018}, read out thousands of channels, and shield the instrumentation from ionizing radiation. In fact, recent research published in Nature suggests that ionizing radiation from cosmic rays and natural radioactivity will be the next limiting factor in qubit coherence \cite{vepsalainen_impact_2020}. Thus, the next leap in QIS will require infrastructure that can successfully operate at sub-Kelvin temperatures at ultra-high vacuum with stringent radiopurity requirements — systems that can be developed by drawing from existing searches for rare-events in nuclear physics such as the search for \ndbd\ with CUPID-1T. 

==> firstspreadsheetlist.tex <==
IJCLab, France	Giuliani	Andrea	andrea.giuliani@IJCLab.in2p3.fr\\
IJCLab, France	Bergé	Laurent	laurent.berge@IJCLab.in2p3.fr\\
IJCLab, France	Bourgeois	Christian	bourgeoi@lal.in2p3.fr\\
IJCLab, France	Chapellier	Maurice	maurice.chapellier@IJCLab.in2p3.fr\\
IJCLab, France	Dumoulin	Louis	louis.dumoulin@IJCLab.in2p3.fr\\
IJCLab, France	Khalife	Hawraa	hawraa.khalife@IJCLab.in2p3.fr\\
IJCLab, France	Guerard	Eric	guerard@lal.in2p3.fr\\
IJCLab, France	Loaiza	Pia	loaiza@lal.in2p3.fr\\
IJCLab, France	Madhukuttan	Madhujith	madhujith.madhukuttan@csnsm.in2p3.fr\\
IJCLab, France	de Marcillac	Pierre	pierre.de-marcillac@IJCLab.in2p3.fr\\
IJCLab, France	Mariam	Riham	riham.mariam@ijclab.in2p3.fr\\
IJCLab, France	Marnieros	Stefanos	stefanos.marnieros@IJCLab.in2p3.fr\\
IJCLab, France	Olivier	Gilles	olivierg@ipno.in2p3.fr\\
IJCLab, France	Olivieri	Emiliano	emiliano.olivieri@IJCLab.in2p3.fr\\
IJCLab, France	Oriol	Christine	christine.oriol@csnsm.in2p3.fr\\
IJCLab, France	Poda	Denys	denys.poda@IJCLab.in2p3.fr\\
IJCLab, France	Redon	Thierry	thierry.redon@IJCLab.in2p3.fr\\
IJCLab, France	Reynet	Denis	reynet@ipno.in2p3.fr\\
IJCLab, France	Scarpaci	Jean-Antoine	jean-antoine.scarpaci@IJCLab.in2p3.fr\\
IJCLab, France	Zolotarova	Anastasiia	anastasiia.zolotarova@IJCLab.in2p3.fr\\
CEA/DRF, France	Nones	Claudia	claudia.nones@cea.fr\\
CEA/DRF, France	Armatol	Antoine	antoine.armatol@cea.fr\\
CEA/DRF, France	Armengaud	Eric	eric.armengaud@cea.fr\\
CEA/DRF, France	Baudin	David	david.baudin@cea.fr\\
CEA/DRF, France	charrier	aurelia	aurelia.charrier@cea.fr\\
CEA/DRF, France	de Combarieu	Matthieu	matthieu.de-combarieu@cea.fr\\
CEA/DRF, France	Ferri	Federico	federico.ferri@cern.ch\\
CEA/DRF, France	Gras	Philippe	philippe.gras@cern.ch\\
CEA/DRF, France	Gros	Michel	michel.gros@cea.fr\\
CEA/DRF, France	Helis	Dounia	dounia.helis@cea.fr\\
CEA/DRF, France	Mauri	Beatrice	beatrice.mauri@cea.fr\\
CEA/DRF, France	Navick	Xavier Francois	navick@cea.fr\\
CEA/DRF, France	Pari	Patrick	patrick.pari@cea.fr\\
CEA/DRF, France	Paul	Bernard	bernard.paul@cea.fr\\
CEA/DRF, France	Tellier	Olivier	olivier.tellier@cea.fr\\
IP2I, France	Gascon	Jules	j.gascon@ipnl.in2p3.fr\\
IP2I, France	Augier	Corinne	c.augier@ipnl.in2p3.fr\\
IP2I, France	Billard	Julien	j.billard@ipnl.in2p3.fr\\
IP2I, France	Cazes	Antoine	a.cazes@ipnl.in2p3.fr\\
IP2I, France	De Jesus	Maryvonne	maryvonn@ipnl.in2p3.fr\\
IP2I, France	Juillard	Alexandre	alexandre.juillard@ipnl.in2p3.fr\\
IP2I, France	Misiak	Dimitri	misiak@ipnl.in2p3.fr\\
IP2I, France	Sanglard	Veronique	sanglard@ipnl.in2p3.fr\\
SIMaP Grenoble, France	Velazquez	Matias	matias.velazquez@grenoble-inp.fr\\
MIB,Italy	Previtali	Ezio	ezio.previtali@mib.infn.it\\
MIB,Italy	Barresi	Andrea	andrea.barresi@mib.infn.it\\
MIB,Italy	Biassoni	Matteo	matteo.biassoni@mib.infn.it\\
MIB,Italy	Branca	Antonio	antonio.branca@pd.infn.it\\
MIB,Italy	Brofferio	Chiara	chiara.brofferio@mib.infn.it\\
MIB,Italy	Capelli	Silvia	silvia.capelli@mib.infn.it\\
MIB,Italy	Carniti	Paolo 	paolo.carniti@mib.infn.it\\
MIB,Italy	Chiesa	Davide	davide.chiesa@mib.infn.it\\
MIB,Italy	Clemenza	Massimiliano	massimiliano.clemenza@mib.infn.it\\
MIB,Italy	Cova	Francesca	francesca.cova@unimib.it\\
MIB,Italy	Cremonesi	Oliviero	oliviero.cremonesi@mib.infn.it\\
MIB,Italy	Fasoli	Mauro	mauro.fasoli@unimib.it\\
MIB,Italy	Faverzani	Marco	marco.faverzani@mib.infn.it\\
MIB,Italy	Ferri	Elena	elena.ferri@mib.infn.it\\
MIB,Italy	Giachero	Andrea	andrea.giachero@mib.infn.it\\
MIB,Italy	Gironi	Luca	luca.gironi@mib.infn.it\\
MIB,Italy	Gotti	Claudio	claudio.gotti@mib.infn.it\\
MIB,Italy	Nastasi	Massimiliano	massimiliano.nastasi@mib.infn.it\\
MIB,Italy	Nutini	Irene 	irene.nutini@gssi.infn.it\\
MIB,Italy	Pavan	Maura	maura.pavan@mib.infn.it\\
MIB,Italy	Pessina	Gianluigi	pessina@mib.infn.it\\
MIB,Italy	Pozzi	Stefano	stefano.pozzi@mib.infn.it\\
MIB,Italy	Previtali	Ezio	ezio.previtali@mib.infn.it\\
MIB,Italy	Sisti	Monica	monica.sisti@mib.infn.it\\
MIB,Italy	Vedda	Anna	anna.vedda@unimib.it\\
Rome, Italy	Cardani	Laura	laura.cardani@roma1.infn.it\\
Rome, Italy	Bellini	Fabio	fabio.bellini@roma1.infn.it\\
Rome, Italy	Casali	Nicola	nicola.casali@roma1.infn.it\\
Rome, Italy	Colantoni	Ivan	ivan.colantoni@cnr.it\\
Rome, Italy	Collamati	Francesco	Francesco.collamati@roma1.infn.it\\
Rome, Italy	Cruciani	Angelo	angelo.cruciani@roma1.infn.it\\
Rome, Italy	D'Imperio	Giulia	giulia.dimperio@roma1.infn.it\\
Rome, Italy	Dafinei	Ioan	ioan.dafinei.@roma1.infn.it\\
Rome, Italy	Fantini	Guido	guido.fantini@roma1.infn.it\\
Rome, Italy	Milana	Silvia	silvia.milana@roma1.infn.it\\
Rome, Italy	Morganti	Silvio	silvio.morganti@roma1.infn.it\\
Rome, Italy	Pettinacci	Valerio	Valerio.pettinacci@roma1.infn.it\\
Rome, Italy	Tomei	Claudia	claudia.tomei@roma1.infn.it\\
LNGS/GSSI, Italy	Bucci	Carlo	carlo.bucci@lngs.infn.it\\
LNGS/GSSI, Italy	Benato	Giovanni	gbenato@berkeley.edu\\
LNGS/GSSI, Italy	Pirro	Stefano	stefano.pirro@lngs.infn.it\\
LNGS/GSSI, Italy	Canonica	Lucia 	lucia.canonica@lngs.infn.it\\
LNGS/GSSI, Italy	Cappelli	Luigi	luigi.cappelli@lngs.infn.it\\
LNGS/GSSI, Italy	Caracciolo	Vincenzo	vincenzo.caracciolo@lngs.infn.it\\
LNGS/GSSI, Italy	Copello	Simone	simone.copello@lngs.infn.it\\
LNGS/GSSI, Italy	D'Addabbo	Antonio	antonio.daddabbo@lngs.infn.it\\
LNGS/GSSI, Italy	Dompe	Valentina	valentina.dompe@gssi.it\\
LNGS/GSSI, Italy	Ferroni	Fernando	fernando.ferroni@roma1.infn.it\\
LNGS/GSSI, Italy	Gorla	Paolo 	paolo.gorla@lngs.infn.it\\
LNGS/GSSI, Italy	Nisi	Stefano	stefano.nisi@lngs.infn.it\\
LNGS/GSSI, Italy	Pagliarone	Carmine	carmine.pagliarone@lngs.infn.it\\
LNGS/GSSI, Italy	Pagnanini	Lorenzo	lorenzo.pagnanini@lngs.infn.it\\
LNGS/GSSI, Italy	Pattavina	Luca	luca.pattavina@lngs.infn.it\\
LNGS/GSSI, Italy	Puiu	Andrei	andrei.puiu@mib.infn.it\\
LNGS/GSSI, Italy	Schaffner	Karoline	karoline.schaeffner@lngs.infn.it\\
Bologna,Italy	Zucchelli	Stefano	stefano.zucchelli@bo.infn.it\\
Bologna,Italy	Moggi	Niccolò	moggi@bo.infn.it\\
LNF,Italy	Franceschi	Alberto	alberto.franceschi@lnf.infn.it\\
LNF,Italy	Napolitano	Tommaso	tommaso.napolitano@lnf.infn.it\\
LNL,Italy	Keppel	Giorgio	giorgio.keppel@lnl.infn.it\\
LNL,Italy	Azzolini	Oscar	oscar.azzolini@lnl.infn.it\\
LNL,Italy	Pira	Cristian	pira.cristian@lnl.infn.it\\
LNL,Italy	Andrii	Tsymbaliuk	Andrii.Tsymbaliuk@lnl.infn.it\\
PD,Italy	Taffarello	Luca	luca.taffarello@pd.infn.it\\
GE,Italy	Di Domizio	Sergio	sergio.didomizio@ge.infn.it\\
GE,Italy	Caminata	Alessio	alessio.caminata@ge.infn.it\\
GE,Italy	Pallavicni	Marco	marco.pallavicini@mib.infn.it\\
CNR-IMM Italy,	Rizzoli	Rita	rizzoli@bo.imm.cnr.it\\
CNR-IMM Italy,	Mancarella	Fulvio	mancarella@bo.imm.cnr.it\\
CNR-IMM Italy,	Boldrini	Virginia	boldrini@bo.imm.cnr.it\\
University of Zaragoza,Spain	Martinez	Maria	mariam@unizar.es\\
INR NASU, Ukraine	Danevich	Fedor	danevich@kinr.kiev.ua\\
INR NASU, Ukraine	Tretyak	Vladimir	tretyak@kinr.kiev.ua\\
INR NASU, Ukraine	Kobychev	Vladislav	kobychev@kinr.kiev.ua\\
INR NASU, Ukraine	Polischuk	Oksana	polischuk@kinr.kiev.ua\\
INR NASU, Ukraine	Zarytskyy	Mykola	zaritsky96@gmail.com\\
ITEP, Russia	Barabash	Alexander	barabash@itep.ru\\
ITEP, Russia	Konovalov	Sergey	konovalov@itep.ru\\
ITEP, Russia	Yumatov	Vladimir	yumatov@itep.ru\\
NIIC, Russia	Shlegel	Vladimir	shlegel@niic.nsc.ru\\
MIT, US	Winslow	Lindley	lwinslow@mit.edu\\
MIT, US	Johnston	Joseph	jpj13@mit.edu\\
MIT, US	Ouellet	Jonathan	ouelletj@mit.edu\\
MIT, US	Formaggio	Joseph	josephf@MIT.EDU\\
UCB/LBNL, US	Kolomensky	Yury	ygkolomensky@lbl.gov\\
UCB/LBNL, US	Beretta	Mattia	mattia.beretta@berkeley.edu\\
UCB/LBNL, US	Dixon	Toby	tdixon@berkeley.edu\\
UCB/LBNL, US	Drobizhev	Alexey	adrobizhev@lbl.gov\\
UCB/LBNL, US	Fujikawa	Brian	BKFujikawa@lbl.gov\\
UCB/LBNL, US	Hansen	Erin	evhansen@berkeley.edu\\
UCB/LBNL, US	Huang	Roger	roger\_huang@berkeley.edu\\
UCB/LBNL, US	Li	Charles	charstnut@berkeley.edu\\
UCB/LBNL, US	Marini	Laura	lmarini@berkeley.edu\\
UCB/LBNL, US	Mei	Yuan	YMei@lbl.gov\\
UCB/LBNL, US	Norman	Eric	EBNorman@lbl.gov\\
UCB/LBNL, US	Sakai	Michinari	michsakai@berkeley.edu\\
UCB/LBNL, US	Schmidt	Benjamin	BESchmidt@lbl.gov\\
UCB/LBNL, US	Singh	Vivek	singhv@berkeley.edu\\
UCB/LBNL, US	Vetter	Kenneth	kenneth\_vetter@berkeley.edu\\
UCB/LBNL, US	Wagaarachchi	Sachi	sachi@berkeley.edu\\
UCB/LBNL, US	Wallig	Joe	\\
UCB/LBNL, US	Welliver	Bradford	bcwelliver@lbl.gov\\
Yale, US	Heeger	Karsten	karsten.heeger@yale.edu\\
Yale, US	Maruyama	Reina	reina.maruyama@yale.edu\\
Yale, US	Nikkel	James	james.nikkel@yale.edu\\
Yale, US	Surukuchi	Pranava Teja 	pranavateja.surukuchi@yale.edu\\
Yale, US	Pagan	Samantha	samantha.pagan@yale.edu\\
ANL, US	Novosad	Valentine	novosad@anl.gov\\
ANL, US	Chang	Clarence	clchang@anl.gov\\
ANL, US	Wang	Gensheng	gwang@anl.gov\\
ANL, US	Pearson	John	\\
ANL, US	Polakovic	T.	tpolakovic@anl.gov\\
ANL, US	Armstrong	W.R. 	warmstrong@anl.gov\\
ANL, US	Yefremenko	V.	yefremenko@anl.gov\\
ANL, US	Zhang	Jianjie	jianjie.zhang@anl.gov\\ 
South Carolina, US	Avignone	Frank	titus3@mac.com\\
South Carolina, US	Creswick	Richard	creswick.rj@sc.edu\\
South Carolina, US	Rusconi	Claudia	claudia.rusconi@lngs.infn.it\\
South Carolina, US	Rosenfeld	Carl	lcr@sc.edu\\
South Carolina, US	Wilson	Jeffry	jwilson@sc.edu\\
South Carolina, US	Wilson	Kevin	kpwilson@pm.me\\
Virginia Tech, US	O'Donnell	Thomas	tdonnell@vt.edu\\
Virginia Tech, US	Dell'Oro	Stefano	sdelloro@vt.edu\\
Cal Poly, US	Gutierrez	Thomas	tdgutier@calpoly.edu\\
Johns Hopkins	Speller	Danielle	dspelle1@jhu.edu\\
CUPID-China, China	Huang	Huan Zhong	huang@physics.ucla.edu\\
USTC	Peng 	Haiping	penghp@ustc.edu.cn\\
USTC	Xue	Mingxuan	xuemx@mail.ustc.edu.cn\\
Fudan-China	Ma	Long	malong@fudan.edu.cn\\
Fudan-China	Shen	Yang	shenyang@fudan.edu.cn\\
Fudan-China	He	Wanbing	hewanbing@fudan.edu.cn\\
Fudan-China	Fu	Shihong	Shihong.Fu@mib.infn.it\\
Shanghai-China	Han	Ke 	ke.han@sjtu.edu.cn\\


==> oldauthlists/cupid_authors.tex <==
\author{A.~Armatol\thanksref{CEA_IRFU_France}
\and
C.~Augier\thanksref{IP2I_France}
\and
F.~T.~Avignone~III\thanksref{UofSC_US}
\and
O.~Azzolini\thanksref{LNL_Italy}
\and
M.~Balata\thanksref{LNGS_Italy}
\and
K.~Ballen\thanksref{LNL_Italy}
\and
A.~S.~Barabash\thanksref{ITEP_Russia}
\and
G.~Bari\thanksref{SdB_Italy}
\and
A.~Barresi\thanksref{MIB_Italy,UniMIB_Italy}
\and
D.~Baudin\thanksref{CEA_IRFU_France}
\and
F.~Bellini\thanksref{SdR_Italy,SURome_Italy}
\and
G.~Benato\thanksref{LNGS_Italy}
\and
M.~Beretta\thanksref{UCB_US}
\and
M.~Bettelli\thanksref{CNR-IMM_Italy}
\and
M.~Biassoni\thanksref{MIB_Italy}
\and
J.~Billard\thanksref{IP2I_France}
\and
V.~Boldrini\thanksref{CNR-IMM_Italy,SdB_Italy}
\and
A.~Branca\thanksref{MIB_Italy,UniMIB_Italy}
\and
C.~Brofferio\thanksref{MIB_Italy,UniMIB_Italy}
\and
C.~Bucci\thanksref{LNGS_Italy}
\and
J.~Camilleri\thanksref{VT_US}
\and
C.~Capelli\thanksref{LBNL_US}
\and
S.~Capelli\thanksref{MIB_Italy,UniMIB_Italy}
\and
L.~Cappelli\thanksref{LNGS_Italy}
\and
L.~Cardani\thanksref{SdR_Italy}
\and
P.~Carniti\thanksref{MIB_Italy,UniMIB_Italy}
\and
N.~Casali\thanksref{SdR_Italy}
\and
E.~Celi\thanksref{LNGS_Italy,GSSI}
\and
C.~Chang\thanksref{ANL_US}
\and
D.~Chiesa\thanksref{MIB_Italy,UniMIB_Italy}
\and
M.~Clemenza\thanksref{MIB_Italy,UniMIB_Italy}
\and
I.~Colantoni\thanksref{CNR-NANOTEC,SdR_Italy}
\and
S.~Copello\thanksref{SdG_Italy,UnivGenova}
\and
E.~Craft\thanksref{Yale_US}
\and
O.~Cremonesi\thanksref{MIB_Italy}
\and
R.~J.~Creswick\thanksref{UofSC_US}
\and
A.~Cruciani\thanksref{SdR_Italy}
\and
A.~D'Addabbo\thanksref{LNGS_Italy}
\and
G.~D'Imperio\thanksref{SdR_Italy}
\and
S.~Dabagov\thanksref{LNF_Italy}
\and
I.~Dafinei\thanksref{SdR_Italy}
\and
F.~A.~Danevich\thanksref{INR_NASU_Ukraine}
\and
M.~De~Jesus\thanksref{IP2I_France}
\and
P.~de~Marcillac\thanksref{IJCLab_France}
\and
S.~Dell'Oro\thanksref{MIB_Italy,UniMIB_Italy}
\and
S.~Di~Domizio\thanksref{SdG_Italy,UnivGenova}
\and
S.~Di~Lorenzo\thanksref{LNGS_Italy}
\and
T.~Dixon\thanksref{IJCLab_France}
\and
V.~Domp\`e\thanksref{SdR_Italy,SURome_Italy}
\and
A.~Drobizhev\thanksref{LBNL_US}
\and
L.~Dumoulin\thanksref{IJCLab_France}
\and
G.~Fantini\thanksref{SdR_Italy,SURome_Italy}
\and
M.~Faverzani\thanksref{MIB_Italy,UniMIB_Italy}
\and
E.~Ferri\thanksref{MIB_Italy,UniMIB_Italy}
\and
F.~Ferri\thanksref{CEA_IRFU_France}
\and
F.~Ferroni\thanksref{SdR_Italy,SURome_Italy,GSSI}
\and
E.~Figueroa-Feliciano\thanksref{NWU_US}
\and
L.~Foggetta\thanksref{LNF_Italy}
\and
J.~Formaggio\thanksref{MIT_US}
\and
A.~Franceschi\thanksref{LNF_Italy}
\and
C.~Fu\thanksref{Fudan-China}
\and
S.~Fu\thanksref{Fudan-China}
\and
B.~K.~Fujikawa\thanksref{LBNL_US}
\and
A.~Gallas\thanksref{IJCLab_France}
\and
J.~Gascon\thanksref{IP2I_France}
\and
S.~Ghislandi\thanksref{GSSI,LNGS_Italy}
\and
A.~Giachero\thanksref{MIB_Italy,UniMIB_Italy}
\and
A.~Gianvecchio\thanksref{MIB_Italy,UniMIB_Italy}
\and
L.~Gironi\thanksref{MIB_Italy,UniMIB_Italy}
\and
A.~Giuliani\thanksref{IJCLab_France}
\and
P.~Gorla\thanksref{LNGS_Italy}
\and
C.~Gotti\thanksref{MIB_Italy}
\and
C.~Grant\thanksref{BU_US}
\and
P.~Gras\thanksref{CEA_IRFU_France}
\and
P.~V.~Guillaumon\thanksref{LNGS_Italy}
\and
T.~D.~Gutierrez\thanksref{CalPoly_US}
\and
K.~Han\thanksref{Shanghai_JTU_China}
\and
E.~V.~Hansen\thanksref{UCB_US}
\and
K.~M.~Heeger\thanksref{Yale_US}
\and
D.~L.~Helis\thanksref{GSSI,LNGS_Italy,e1}
%\and
%D.~L.~Helis\thanksref{CEA_IRFU_France}
\and
H.~Z.~Huang\thanksref{UCLA_US,Fudan-China}
\and
R.~G.~Huang\thanksref{UCB_US,LBNL_US}
\and
L.~Imbert\thanksref{IJCLab_France}
\and
J.~Johnston\thanksref{MIT_US}
\and
A.~Juillard\thanksref{IP2I_France}
\and
G.~Karapetrov\thanksref{Drexel_US}
\and
G.~Keppel\thanksref{LNL_Italy}
\and
H.~Khalife\thanksref{CEA_IRFU_France}
\and
V.~V.~Kobychev\thanksref{INR_NASU_Ukraine}
\and
Yu.~G.~Kolomensky\thanksref{UCB_US,LBNL_US}
\and
S.~I.~Konovalov\thanksref{ITEP_Russia}
\and
R.~Kowalski\thanksref{JHU_US}
\and
T.~Langford\thanksref{Yale_US}
\and
M.~Lefevre1\thanksref{CEA_IRFU_France}
\and
R.~Liu\thanksref{Yale_US}
\and
Y.~Liu\thanksref{BNU-China}
\and
P.~Loaiza\thanksref{IJCLab_France}
\and
L.~Ma\thanksref{Fudan-China}
\and
M.~Madhukuttan\thanksref{IJCLab_France}
\and
F.~Mancarella\thanksref{CNR-IMM_Italy,SdB_Italy}
\and
L.~Marini\thanksref{LNGS_Italy,GSSI}
\and
S.~Marnieros\thanksref{IJCLab_France}
\and
M.~Martinez\thanksref{Zaragoza,ARAID}
\and
R.~H.~Maruyama\thanksref{Yale_US}
\and
Ph.~Mas\thanksref{CEA_IRFU_France}
\and
B.~Mauri\thanksref{CEA_IRFU_France}
\and
D.~Mayer\thanksref{MIT_US}
\and
G.~Mazzitelli\thanksref{LNF_Italy}
\and
Y.~Mei\thanksref{LBNL_US}
\and
S.~Milana\thanksref{SdR_Italy}
\and
S.~Morganti\thanksref{SdR_Italy}
\and
T.~Napolitano\thanksref{LNF_Italy}
\and
M.~Nastasi\thanksref{MIB_Italy,UniMIB_Italy}
\and
J.~Nikkel\thanksref{Yale_US}
\and
S.~Nisi\thanksref{LNGS_Italy}
\and
C.~Nones\thanksref{CEA_IRFU_France}
\and
E.~B.~Norman\thanksref{UCB_US}
\and
V.~Novosad\thanksref{ANL_US}
\and
I.~Nutini\thanksref{MIB_Italy,UniMIB_Italy}
\and
T.~O'Donnell\thanksref{VT_US}
\and
E.~Olivieri\thanksref{IJCLab_France}
\and
M.~Olmi\thanksref{LNGS_Italy}
\and
J.~L.~Ouellet\thanksref{MIT_US}
\and
S.~Pagan\thanksref{Yale_US}
\and
C.~Pagliarone\thanksref{LNGS_Italy}
\and
L.~Pagnanini\thanksref{LNGS_Italy,GSSI}
\and
L.~Pattavina\thanksref{LNGS_Italy}
\and
M.~Pavan\thanksref{MIB_Italy,UniMIB_Italy}
\and
H.~Peng\thanksref{USTC}
\and
G.~Pessina\thanksref{MIB_Italy}
\and
V.~Pettinacci\thanksref{SdR_Italy}
\and
C.~Pira\thanksref{LNL_Italy}
\and
S.~Pirro\thanksref{LNGS_Italy}
\and
D.~V.~Poda\thanksref{IJCLab_France}
\and
O.~G.~Polischuk\thanksref{INR_NASU_Ukraine}
\and
I.~Ponce\thanksref{Yale_US}
\and
S.~Pozzi\thanksref{MIB_Italy,UniMIB_Italy}
\and
E.~Previtali\thanksref{MIB_Italy,UniMIB_Italy}
\and
A.~Puiu\thanksref{LNGS_Italy,GSSI}
\and
S.~Quitadamo\thanksref{GSSI,LNGS_Italy}
\and
A.~Ressa\thanksref{SdR_Italy,SURome_Italy}
\and
R.~Rizzoli\thanksref{CNR-IMM_Italy,SdB_Italy}
\and
C.~Rosenfeld\thanksref{UofSC_US}
\and
P.~Rosier\thanksref{IJCLab_France}
\and
J.~A.~Scarpaci\thanksref{IJCLab_France}
\and
B.~Schmidt\thanksref{NWU_US,LBNL_US}
\and
V.~Sharma\thanksref{VT_US}
\and
V.~Shlegel\thanksref{NIIC_Russia}
\and
V.~Singh\thanksref{UCB_US}
\and
M.~Sisti\thanksref{MIB_Italy}
\and
P.~Slocum\thanksref{Yale_US}
\and
D.~Speller\thanksref{JHU_US,Yale_US}
\and
P.~T.~Surukuchi\thanksref{Yale_US}
\and
L.~Taffarello\thanksref{PD_Italy}
\and
C.~Tomei\thanksref{SdR_Italy}
\and
J.~Torres\thanksref{Yale_US}
\and
V.~I.~Tretyak\thanksref{INR_NASU_Ukraine}
\and
A.~Tsymbaliuk\thanksref{LNL_Italy}
\and
M.~Velazquez\thanksref{SIMaP_Grenoble_France}
\and
K.~J.~Vetter\thanksref{UCB_US}
\and
S.~L.~Wagaarachchi\thanksref{UCB_US}
\and
G.~Wang\thanksref{ANL_US}
\and
L.~Wang\thanksref{BNU-China}
\and
R.~Wang\thanksref{JHU_US}
\and
B.~Welliver\thanksref{UCB_US,LBNL_US}
\and
J.~Wilson\thanksref{UofSC_US}
\and
K.~Wilson\thanksref{UofSC_US}
\and
L.~A.~Winslow\thanksref{MIT_US}
\and
M.~Xue\thanksref{USTC}
\and
L.~Yan\thanksref{Fudan-China}
\and
J.~Yang\thanksref{USTC}
\and
V.~Yefremenko\thanksref{ANL_US}
\and
V.~I.~Umatov\thanksref{ITEP_Russia}
\and
M.~M.~Zarytskyy\thanksref{INR_NASU_Ukraine}
\and
J.~Zhang\thanksref{ANL_US}
\and
A.~S.~Zolotarova\thanksref{CEA_IRFU_France,e2}
\and
S.~Zucchelli\thanksref{SdB_Italy,UnivBologna_Italy}
}

\institute{IRFU, CEA, Universit\'e Paris-Saclay, Saclay, France\label{CEA_IRFU_France}
\and
Univ Lyon, Université Lyon 1, CNRS/IN2P3, IP2I, Lyon, France\label{IP2I_France}
\and
University of South Carolina, Columbia, SC, USA\label{UofSC_US}
\and
INFN Laboratori Nazionali di Legnaro, Legnaro, Italy\label{LNL_Italy}
\and
INFN Laboratori Nazionali del Gran Sasso, Assergi (AQ), Italy\label{LNGS_Italy}
\and
National Research Centre Kurchatov Institute, Institute for Theoretical and Experimental Physics, Moscow, Russia\label{ITEP_Russia}
\and
INFN Sezione di Bologna, Bologna, Italy\label{SdB_Italy}
\and
INFN Sezione di Milano - Bicocca, Milano, Italy\label{MIB_Italy}
\and
University of Milano - Bicocca, Milano, Italy\label{UniMIB_Italy}
\and
INFN Sezione di Roma, Rome, Italy\label{SdR_Italy}
\and
Sapienza University of Rome, Rome, Italy\label{SURome_Italy}
\and
University of California, Berkeley, CA, USA\label{UCB_US}
\and
CNR-Institute for Microelectronics and Microsystems, Bologna, Italy\label{CNR-IMM_Italy}
\and
Virginia Polytechnic Institute and State University, Blacksburg, VA, USA\label{VT_US}
\and
Lawrence Berkeley National Laboratory, Berkeley, CA, USA\label{LBNL_US}
\and
Gran Sasso Science Institute, L'Aquila, Italy\label{GSSI}
\and
Argonne National Laboratory, Argonne, IL, USA\label{ANL_US}
\and
CNR-Institute of Nanotechnology, Rome, Italy\label{CNR-NANOTEC}
\and
INFN Sezione di Genova, Genova, Italy\label{SdG_Italy}
\and
University of Genova, Genova, Italy\label{UnivGenova}
\and
Yale University, New Haven, CT, USA\label{Yale_US}
\and
INFN Laboratori Nazionali di Frascati, Frascati, Italy\label{LNF_Italy}
\and
Institute for Nuclear Research of NASU, Kyiv, Ukraine\label{INR_NASU_Ukraine}
\and
Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\label{IJCLab_France}
\and
Northwestern University, Evanston, IL, USA\label{NWU_US}
\and
Massachusetts Institute of Technology, Cambridge, MA, USA\label{MIT_US}
\and
Fudan University, Shanghai, China\label{Fudan-China}
\and
Boston University, Boston, MA, USA\label{BU_US}
\and
California Polytechnic State University, San Luis Obispo, CA, USA\label{CalPoly_US}
\and
Shanghai Jiao Tong University, Shanghai, China\label{Shanghai_JTU_China}
\and
University of California, Los Angeles, CA, USA\label{UCLA_US}
\and
Drexel University, Philadelphia, PA, USA\label{Drexel_US}
\and
Johns Hopkins University, Baltimore, MD, USA\label{JHU_US}
\and
Beijing Normal University, Beijing, China\label{BNU-China}
\and
Centro de Astropart{\'\i}culas y F{\'\i}sica de Altas Energ{\'\i}as, Universidad de Zaragoza, Zaragoza, Spain\label{Zaragoza}
\and
ARAID Fundaci\'on Agencia Aragonesa para la Investigaci\'on y el Desarrollo, Zaragoza, Spain\label{ARAID}
\and
University of Science and Technology of China, Hefei, China\label{USTC}
\and
Nikolaev Institute of Inorganic Chemistry, Novosibirsk, Russia\label{NIIC_Russia}
\and
INFN Sezione di Padova, Padova, Italy\label{PD_Italy}
\and
Univ. Grenoble Alpes, CNRS, Grenoble INP, SIMAP, Grenoble, France\label{SIMaP_Grenoble_France}
\and
University of Bologna, Bologna, Italy\label{UnivBologna_Italy}
}

\thankstext{e1}{Previously at: IRFU, CEA, Universit\'e Paris-Saclay, Saclay, France}
\thankstext{e2}{Presently at: IRFU, CEA, Universit\'e Paris-Saclay, Saclay, France}

==> oldauthlists/cupid_collaboration_auth_june2021doeprop_modified.tex <==
\section{CUPID Collaboration and Project Team }
\label{sec:cupid-collaboration}

The CUPID Collaboration and Project Team including both physics and technical authors is a robust international collaboration that brings together an array of experts that will contribute to a successful program.\\

\noindent
{\bf IRFU, CEA, Universit\'e Paris-Saclay, Saclay, France}\\
A.~Armatol, D.~Baudin, F.~Ferri, P.~Gras, D.~L.~Helis, H.~Khalife, B.~Mauri, C.~Nones\\
\\
{\bf Institut de Physique des 2 Infinis, Lyon, France}\\
C.~Augier, J.~Billard, M.~De~Jesus, J.~Gascon, A.~Juillard\\
\\
{\bf University of South Carolina, Columbia, SC, USA}\\
F.~T.~Avignone~III, R.~J.~Creswick, K.~Wilson\\
\\
{\bf INFN Laboratori Nazionali di Legnaro, Legnaro, Italy}\\
O.~Azzolini, K.~Ballen, G.~Keppel, C.~Pira, A.~Tsymbaliuk\\
\\
{\bf National Research Centre Kurchatov Institute, Institute for Theoretical and Experimental Physics, Moscow, Russia}\\
A.S.~Barabash, S.I.~Konovalov, V.I.~Umatov\\
\\
{\bf INFN Sezione di Bologna, Bologna, Italy}\\
G.~Bari, S.~Zucchelli\\
\\
{\bf INFN Sezione di Milano - Bicocca, Milano, Italy}\\
A.~Barresi, M.~Biassoni, A.~Branca, C.~Brofferio, S.~Capelli, P.~Carniti, D.~Chiesa, M.~Clemenza, O.~Cremonesi, S.~Dell'Oro, M.~Faverzani, E.~Ferri, A.~Giachero, L.~Gironi, C.~Gotti, M.~Nastasi, I.~Nutini, M.~Pavan, G.~Pessina, S.~Pozzi, E.~Previtali, M.~Sisti\\
\\
{\bf INFN Sezione di Roma, Rome, Italy}\\
F.~Bellini, L.~Cardani, N.~Casali, I.~Colantoni, A.~Cruciani, G.~D'Imperio, I.~Dafinei, V.~Domp\`e, G.~Fantini, F.~Ferroni, S.~Milana, V.~Pettinacci, A.~Ressa, C.~Tomei\\
\\
{\bf INFN Laboratori Nazionali del Gran Sasso, Assergi (AQ), Italy}\\
G.~Benato, C.~Bucci, L.~Cappelli, E.~Celi, A.~D'Addabbo, P.~Gorla, L.~Marini, S.~Nisi, C.~Pagliarone, L.~Pagnanini, L.~Pattavina, S.~Pirro, A.~Puiu\\
\\
{\bf University of California, Berkeley, CA, USA}\\
M.~Beretta, E.~V.~Hansen, R.~G.~Huang, Yu.~G.~Kolomensky, E.~B.~Norman, V.~Singh, K.~J.~Vetter, S.~L.~Wagaarachchi\\
\\
{\bf Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France}\\
L.~Berg\'e, P.~de~Marcillac, L.~Dumoulin, A.~Gallas, A.~Giuliani, E.~Guerard, L.~Imbert, P.~Loaiza, M.~Madhukuttan, S.~Marnieros, E.~Olivieri, D.~V.~Poda, T.~Redon, P.~Rosier, J.~Scarpaci, A.~Zolotarova\\
\\
{\bf CNR-Institute for Microelectronics and Microsystems, Bologna, Italy}\\
V.~Boldrini, F.~Mancarella, R.~Rizzoli\\
\\
{\bf Lawrence Berkeley National Laboratory, Berkeley, CA, USA}\\
J.~Bramble, C.~Capelli, A.~Drobizhev, A.~Emmanuel, B.~K.~Fujikawa, Y.~Mei, T.~Stezelberger, J.~G.~Wallig, B.~Welliver\\
\\
{\bf Virginia Polytechnic Institute and State University, Blacksburg, VA, USA}\\
J.~Camilleri, T.~O'Donnell, V.~Sharma\\
\\
{\bf Argonne National Laboratory, Argonne, IL, USA}\\
C.~Chang, M.~Lisovenko, V.~Novosad, J.~Pearson, G.~Wang, V.~Yefremenko, J.~Zhang\\
\\
{\bf INFN Sezione di Genova, Genova, Italy}\\
S.~Copello, S.~Di~Domizio\\
\\
{\bf Institute for Nuclear Research of NASU, Kyiv, Ukraine}\\
F.~A.~Danevich, V.~V.~Kobychev, O.~G.~Polischuk, V.~I.~Tretyak, M.~M.~Zarytskyy\\
\\
{\bf Northwestern University, Evanston, IL, USA}\\
E.~Figueroa-Feliciano, B.~Schmidt\\
\\
{\bf Massachusetts Institute of Technology, Cambridge, MA, USA}\\
J.~Formaggio, J.~Johnston, D.~Mayer, J.~L.~Ouellet, L.~A.~Winslow\\
\\
{\bf INFN Laboratori Nazionali di Frascati, Frascati, Italy}\\
A.~Franceschi, T.~Napolitano\\
\\
{\bf Fudan University, Shanghai, China}\\
C.~Fu, S.~Fu, L.~Ma, L.~Yan\\
\\
{\bf Boston University, Boston, MA, USA}\\
C.~Grant\\
\\
{\bf California Polytechnic State University, San Luis Obispo, CA, USA}\\
T.~D.~Gutierrez\\
\\
{\bf Shanghai Jiao Tong University, Shanghai, China}\\
K.~Han\\
\\
{\bf Yale University, New Haven, CT, USA}\\
K.~M.~Heeger, R.~Liu, R.~H.~Maruyama, J.~Nikkel, S.~Pagan, I.~Ponce, P.~Slocum, P.~T.~Surukuchi, J.~A.~Torres, J.~Wilhelmi\\
\\
{\bf University of California, Los Angeles, CA, USA}\\
H.~Z.~Huang\\
\\
{\bf Drexel University, Philadelphia, PA, USA}\\
G.~Karapetrov\\
\\
{\bf Beijing Normal University, Beijing, China}\\
Y.~Liu, L.~Wang\\
\\
{\bf Centro de Astropart{\'\i}culas y F{\'\i}sica de Altas Energ{\'\i}as, Universidad de Zaragoza, Zaragoza, Spain}\\
M.~Martinez, A.~Ortiz~de~Solorzano\\
\\
{\bf University of Science and Technology of China, Hefei, China}\\
H.~Peng, M.~Xue, J.~Yang\\
\\
{\bf Nikolaev Institute of Inorganic Chemistry, Novosibirsk, Russia}\\
V.~Shlegel\\
\\
{\bf Johns Hopkins University, Baltimore, MD, USA}\\
D.~Speller, R. Kowalski\\
\\
{\bf INFN Sezione di Padova, Padova, Italy}\\
L.~Taffarello\\
\\
{\bf Laboratoire de Science et Ing\'enierie des Mat\'eriaux et Proc\'ed\'es, Grenoble, France}\\
M.~Velazquez\\

